Interact as You Intend: Intention-Driven Human-Object Interaction Detection

The recent advances in instance-level detection tasks lay strong foundation for genuine comprehension of the visual scenes. However, the ability to fully comprehend a social scene is still in its preliminary stage. In this work, we focus on detecting human-object interactions (HOIs) in social scene images, which is demanding in terms of research and increasingly useful for practical applications. To undertake social tasks interacting with objects, humans direct their attention and move their body based on their intention. Based on this observation, we provide a unique computational perspective to explore human intention in HOI detection. Specifically, the proposed human intention-driven HOI detection (iHOI) framework models human pose with the relative distances from body joints to the object instances. It also utilizes human gaze to guide the attended contextual regions in a weakly-supervised setting. In addition, we propose a hard negative sampling strategy to address the problem of mis-grouping. We perform extensive experiments on two benchmark datasets, namely V-COCO and HICO-DET. The efficacy of each proposed component has also been validated.

==> table/fig_multiact_multiobj.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=1.0\linewidth]{multiact_multiobj.pdf}
%	\begin{minipage}{1.0\columnwidth}
%  	\begin{minipage}{0.515\columnwidth}
%		 	\centerline{\includegraphics[width=1.0\linewidth]{multiact_sample_1}}
%		 	\centerline{\includegraphics[width=1.0\linewidth]{multiobj_sample_2}}
%  	\end{minipage}
%  	\hfill
%  	\begin{minipage}{0.474\columnwidth}
%		 	\centerline{\includegraphics[width=1.0\linewidth]{multiact_sample_2}}
%		 	\centerline{\includegraphics[width=1.0\linewidth]{multiobj_sample_1}}
%  	\end{minipage}
%  \end{minipage}
	\vspace{-2ex}
	\caption
		{
		%\small
		Our method addresses the following two scenarios: 
		the first row shows that human can perform multiple actions on a targeting object;
		the second row shows that a person can perform the same action on multiple objects simultaneously.
		} 
\label{fig:multiact_multiobj}
\end{figure}

==> table/fig_size.tex <==
\begin{figure}[!htbp]
	\centering
	\includegraphics[width=0.5\linewidth]{size_effect.pdf}
	\caption
		{
        Ablation on V-COCO dataset: candidate region selection effect on mAP(\%).
		} 
	\vspace{-1ex}
\label{fig:size}
\end{figure}
